Natural Language Decompositions of Implicit Content Enable Better Text Representations

When people interpret text, they rely on inferences that go beyond the observed language itself. Inspired by this observation, we introduce a method for the analysis of text that takes implicitly communicated content explicitly into account. We use a large language model to produce sets of propositions that are inferentially related to the text that has been observed, then validate the plausibility of the generated content via human judgments. Incorporating these explicit representations of implicit content proves useful in multiple problem settings that involve the human interpretation of utterances: assessing the similarity of arguments, making sense of a body of opinion data, and modeling legislative behavior. Our results suggest that modeling the meanings behind observed language, rather than the literal text alone, is a valuable direction for NLP and particularly its applications to social science.

==> Decompositions_as_First_Class_Citizens_arXiv/sections/00-abstract.tex <==
When people interpret text, they rely on inferences that go beyond the observed language itself. Inspired by this observation, we introduce a method for the analysis of text that takes implicitly communicated content explicitly into account. We use a large language model to produce sets of propositions that are inferentially related to the text that has been observed, then validate the plausibility of the generated content via human judgments.
Incorporating these explicit representations of implicit content proves useful in multiple problem settings that involve the human interpretation of utterances: assessing the similarity of arguments, making sense of a body of opinion data, and modeling legislative behavior. Our results suggest that modeling the meanings behind observed language, rather than the literal text alone, is a valuable direction for NLP and particularly its applications to social science.\footnote{Code and data available at \url{github.com/ahoho/inferential-decompositions}}

==> Decompositions_as_First_Class_Citizens_arXiv/sections/01-intro.tex <==
\section{Introduction}\label{sec:background}

\begin{figure}[!h]
\centering
\includegraphics[scale=0.75]{figures/teaser_figure_cr.pdf}
\caption{Example showing a pair of tweets from legislators along with inferentially-related propositions. Embeddings over observed tweets have a high cosine distance, while embeddings over (different types of) propositions place them closer to each other (see \cref{sec:covote_prediction}).}
\label{fig:teaser}
\vspace{-0.3cm}
\end{figure}

The meaning and import of an utterance are often underdetermined by the utterance itself.
Human interpretation involves making inferences based on the utterance to understand what it communicates \cite{bach1994,hobbs1993interpretation}.
For the disciplines and applications that are concerned with making sense of large amounts of text data, human interpretation of each individual utterance is intractable.
Some NLP methods are designed to facilitate human interpretation of text by aggregating lexical data; for example, dictionaries map words to constructs \cite[e.g.,][]{pennebaker2001linguistic}, and topic models discover interpretable categories in a form of automated qualitative content analysis \cite{Grimmer2013TextAD,hoyle-etal-2022-neural}.
Much of the time, though, these techniques operate over surface forms alone, limiting their ability to capture implicit content that facilitates human interpretation. While contextual embeddings are a step in this direction, these representations remain dominated by lexical content \cite{zhang-etal-2019-paws}.

In this work, we introduce a framework for the interpretation of text data at scale that takes implicitly communicated content more explicitly into account.
Specifically, we generate sets of straightforward propositions that are inferentially related to the original texts.
We refer to these as \emph{inferential decompositions} because they break the interpretations of utterances into smaller units.
Broadly speaking, we follow \citet[][p. 476]{bach2004pragmatics} in distinguishing ``information encoded in what is uttered'' from extralinguistic information.
Rather than being logical entailments, these generations are \emph{plausible entailments} of the kind found in discussions of textual entailment \cite{Dagan2009RecognizingTE} and implicature \cite{sep-implicature}.%
This idea relates to decompositional semantics \cite{white-etal-2020-universal}, but eschews linguistically-motivated annotations in favor of a more open-ended structure that facilitates direct interpretation in downstream applications.

We perform this process using a large language model (LLM), specifying a practitioner protocol for crafting exemplars that capture explicit and implicit propositions based on utterances sampled from the corpus of interest, thereby guiding the language model to do the same (\cref{sec:background}).
In designing our approach, we observe that the inherent sparseness of text data often makes it useful to represent text using lower-dimensional representations. 
Accordingly, our notion of decomposition (and the generation process) encourages propositions that contain simple language, making them both easier to interpret and more amenable to standard embedding techniques.
We observe that the viability of this technique rests on models' ability to reliably generate real-world associations \cite{petroni-etal-2019-language,jiang-etal-2020-know,Patel2022MappingLM}, as well as their capacity to follow instructions and mirror the linguistic patterns of provided exemplars \cite{brown2020language,liu-etal-2022-wanli}.%

We situate our approach within the \emph{text-as-data} framework: the ``systematic analysis of large-scale text collections'' that can help address substantive problems within a particular discipline \cite{Grimmer2013TextAD}.
First, we validate our method with human annotations, verifying that generated decompositions are plausible and easy to read, and we also show that embeddings of these inferential decompositions can be used to improve correlation with human judgments of argument similarity  (\cref{sec:validation}).
We then turn to two illustrations of the technique's utility, both drawn from real-world, substantive problems in computational social science. The first problem involves making sense of the space of public opinion, facilitating human interpretation of a set of comments responding to the US Food and Drug Administration's plans to authorize a COVID-19 vaccine for children (\cref{sec:clustering}). The second involves the question of how likely two legislators are to vote together based on their tweets  (\cref{sec:covote_prediction}).


==> Decompositions_as_First_Class_Citizens_arXiv/sections/02-background.tex <==
\begin{figure}[ht]
  \centering
  \begin{minipage}{0.48\textwidth}
    \small{\textcolor{britishracinggreen}{\textvtt{Human utterances  communicate propositions that may or may not  be explicit in  the literal meaning of the utterance. For each utterance, state the implicit and explicit propositions communicated by that  utterance in a brief list. Implicit propositions may be inferences about the subject of the utterance or about the perspective of  its author. All generated propositions  should be short, independent, and written in direct speech and simple sentences.}}
    
    \textvtt{\#\#\#}
    
    \textvtt{\textcolor{britishracinggreen}{INPUT:} \textcolor{gray}{\{ utterance \}}}
    
    {\textvtt{\textcolor{britishracinggreen}{OUTPUT:} \textcolor{gray}{\{ inference 1 \} | \{ inference 2 \} | $\ldots$}}}
    }

    
  \end{minipage}
\caption{A condensed version of our prompt to models.}
\vspace{-0.3cm}
\label{fig:prompt}
\end{figure}

\section{The Method and its Rationale}\label{sec:background}


The key idea in our approach is to go beyond the observable text to explicitly represent and use the kinds of implicit content that people use when interpreting text in context.

Consider the sentence \emph{Build the wall!}. Following \citet{bender-koller-2020-climbing}, human interpretation of this sentence in context involves deriving the speaker's communicative intent~$i$ from the expression itself, $e$, together with an implicit universe of propositions \emph{outside} the utterance, $U$---world knowledge, hypotheses about the speaker's beliefs, and more.
In this case, some elements of $U$ might be factual background knowledge such as ``The U.S. shares a border with Mexico'' that is not communicated by $e$ itself. Other elements might include implicitly communicated propositions such as ``immigration should be limited''. Propositions from this latter category, consisting of relevant plausible entailments \emph{from} the utterance, we denote as~$\mathcal{R} \subset U$.\looseness=-1\footnote{Cf. \citeauthor{bach2004pragmatics}'s characterization of pragmatic information as ``relevant to the hearer's determination of what the speaker is communicating ... generated by, or at least made relevant by, the act of uttering it''.
Similarly, interpretation as abduction \cite{hobbs1993interpretation} is an inferential process that starts \emph{from} the utterance.}


We are motivated by the idea that, if human interpretation includes the identification of plausible entailments $\cal{R}$ based on the expressed $e$, automated text analysis can also benefit from such inferences, particularly in scenarios where understanding text goes beyond ``who did what to whom''.
The core of our approach is to take an expression and \emph{explicitly} represent, as language, a body of propositions that are related inferentially to it.%

Operationally, our method is as follows:
\begin{enumerate}[nosep]
    \item For the target dataset, randomly sample a small number of items (e.g., tweets).
    \item Craft explicit and implicit propositions relevant to the items (inferential decompositions expressed as language) following the instructions in \cref{app:meta_prompt} to form exemplars.
    \item Prompt a large language model with our instructions (\cref{fig:prompt}) and these exemplars.
    \item Confirm that a random sample of the generated decompositions are plausible (\cref{sec:validation}).\footnote{While this step is not necessary, we recommend validating generations, particularly in sensitive use cases.}
    \item Use the decompositions in the target task.
    
\end{enumerate}

To ground these propositions in a context, we develop domain-dependent user guidelines (step 2) for exemplar creation, limiting the focus to inferences about the utterance topic and its speaker (and explicit content, \cref{app:meta_prompt}).\footnote{In principle, alternative guidelines meeting other desiderata are possible, and can be validated with the same process.}

Continuing with the example $e$ of \emph{Build the wall!}, the method might generate the augmented representation $\mathcal{R} = \{$\emph{A US border wall will reduce border crossings}, \emph{Illegal immigation should be stopped}, $\ldots \}$ as plausible inferences about the speaker's perspective
(an actual example appears in \cref{fig:teaser}).

Because the propositions are expressed in simple language, they are easier to represent with standard embedding techniques: when using $K$-means clustering to over the embedded representations, the clusters are far more readable and distinct than baselines (\cref{sec:clustering}).
Hence, this approach facilitates interpretation of text data at scale.\footnote{``Scale'' refers to dataset sizes that render human analysis too costly, and is constrained only by computational budget.}

==> Decompositions_as_First_Class_Citizens_arXiv/sections/03-validation.tex <==

\section{Generation Validity}\label{sec:validation}
\begin{figure}[tb]
    \centering
    \includegraphics[width=.95\columnwidth]{figures/generation_validation_barplot.pdf}
    \caption{Human-judged plausibility of inferentially-related propositions for different inference types. The vast majority of inferred propositions are plausible.}
    \label{fig:validation}
    \vspace{-0.3cm}
\end{figure}


\begin{table}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{llrrrr}
\toprule
     &          & \multicolumn{3}{c}{Decompositions} \\
     & Baseline & Explicit & Implicit & Both \\
    \midrule
    \emph{Implicit} & & & & \\
    Arg Facet & 54.01 & \underline{59.98} & \underline{58.84} & \underline{59.79} \\
    BWS Arg. & 53.74 & \underline{55.32} & \underline{54.63} & \underline{55.09} \\
    UKP Aspect & 50.04 & \underline{52.86} & \underline{53.40} & \underline{53.39} \\
    \midrule[0.5pt]
    \emph{Explicit} & & & & \\
    Twitter-STS & 69.05 & \underline{72.69} & \underline{69.92} & \underline{71.92} \\
    SICK-R & 80.59 & \underline{81.39} & 75.92 & 80.00 \\
    STS-B & 83.42 & 81.27 & 77.59 & 81.76 \\
    \bottomrule
    \end{tabular}
}
\caption{Measured against human similarity judgments, similarities computed using inferential decompositions are generally better than similarities computed using the observable text (Spearman $\rho$). Improvements from the baseline are \underline{underlined}.}
\label{tab:arg-sts}
\vspace{-0.3cm}
\end{table}

Text analysis methods used in the computational social sciences have known issues with validity.
The interpretation of unsupervised models is particularly fraught---leading to potentially incorrect inferences about the data under study \cite{Baden2021ThreeGI}.
We validate the two components of our approach: the quality of the generations and the similarity of their embeddings.

 

First, if we want to use the generated inferential decompositions in downstream applications, it is important that they are \emph{reasonable} inferences from the original utterance.
Large language models are known to hallucinate incorrect information in some circumstances \cite{maynez-etal-2020-faithfulness,cao-etal-2022-hallucinated,ji2023survey}, but can also exhibit high factuality relative to prior methods \cite{goyal2023news}.
This leads to the question: \emph{Do language models reliably produce plausible explicit \& implicit propositions?}

Second, since similarity over embedded text underpins both the text analysis (\cref{sec:clustering}) and downstream application (\cref{sec:covote_prediction}) that validate our approach, we measure the correlation of embedding and ground-truth similarities for several standard semantic-textual-similarity tasks.
Assuming that human similarity judgments make use of both explicit and implicit inferences, we also ask \emph{whether including such information in sentence representations improve automated estimates of similarity}.

\paragraph{Generation of decompositions.} We generate inferential decompositions for datasets across a diverse set of domains.
Our method should effectively encode stance, often an implicit property of text, so we adopt three argument similarity datasets (\emph{Argument Facets} from \citealt{misra-etal-2016-measuring}; \emph{BWS} from \citealt{BWS}; and \emph{UKP} from \citealt{reimers-etal-2019-classification}).
As a reference point, we also select several standard STS tasks from the Massive Text Embedding Benchmark, which are evaluated for their observed semantic similarity \cite[MTEB,][]{muennighoff2022mteb}.\footnote{For the Twitter dataset \cite{xu-etal-2015-semeval}, we use the original 5-scale Likert similarity, not the binary scores in MTEB.}
We also use the datasets underpinning our analyses in sections \ref{sec:clustering} and \ref{sec:covote_prediction}: public commentary on FDA authorization of COVID-19 vaccines, and tweets from US senators. %

To generate decompositions, we use the instructions and exemplars in \cref{app:prompts}, further dividing the exemplars into \emph{explicit} and \emph{implicit} categories, as determined by our guidelines (\cref{app:meta_prompt}).
See \cref{fig:teaser} for an illustration.
For the human annotation, we sample 15 examples each from STS-B \cite{cer-etal-2017-semeval}, BWS, Twitter-STS  \cite{xu-etal-2015-semeval}, and our two analysis datasets.
The language model is \texttt{text-davinci-003} \cite[\textsc{InstructGPT},][]{ouyang-etal-2022-instructgpt}, and embeddings use \texttt{all-mpnet-base-v2} \cite{reimers-gurevych-2019-sentence}.
Throughout this work, we use nucleus sampling with $p=0.95$ \cite{Holtzman2019TheCC} and a temperature of 1.



\paragraph{Human annotation of plausiblity.} 
In answering the first question, a set of 80 crowdworkers annotated the extent to which a decomposition is reasonable given an utterance---from ``1 - Definitely'' to ``5 - Definitely not''---and whether it adds new information to that utterance (full instructions in \cref{app:human_annotation_instructions_examples}, recruitment details in \cref{app:survey_details}).
We majority-code both answers, breaking ties for the plausibility scores with the rounded mean.

In the vast majority of cases (85\%-93\%), the generated decompositions are at least ``probably'' reasonable (\cref{fig:validation}).
As expected, the plausibility of \emph{implicit} inferences tends to be less definite than either a paraphrase baseline or explicit inferences---but this also speaks to their utility, as they convey additional information not in the text.
Indeed, implicit inferences add new information 40\% of the time, compared to 7\% for explicit inferences (and 15\% for paraphrases).
As further validation to support the analyses in \cref{sec:covote_prediction}, a professor of political science annotated the implicit decompositions of observable legislative tweets, finding 12 of 15 to be at least ``probably reasonable,'' two ambiguous, and one ``probably not reasonable''.%

\paragraph{Semantic Textual Similarity.} Here, we measure whether our method can improve automated measurements of semantic sextual similarity. 
For each example in each of the STS datasets, we form a set $S_i = \{s_i, \tilde{s}_{i,1}, \tilde{s}_{i,2}, \ldots, \tilde{s}_{i,n}\}$ consisting of the original utterance and $n$~decompositions.
As baseline, we computed the cosine similarity comparisons between embeddings of the original sentences $s_i, s_j$, obtained using \texttt{all-mpnet-base-v2}.
Pairwise comparisons for expanded representations $S_i, S_j$, were scored by concatenating the embedding for $s_i$ with the mean of the embeddings for the $s_{i,*}$.\footnote{Approaches designed to measure the similarity of sets of vectors gave similar results\cite[e.g.,][]{zhelezniak-etal-2020-estimating}}

Our method substantially improves correlation on the argument similarity datasets over the embedding baseline (\cref{tab:arg-sts}), where pairs are annotated for the similarity of their position and explanation with respect to a particular topic (e.g., supporting a minimum wage increase by invoking inflation).
In this task, explicit decompositions resemble the implicit ones---annotators give similar proportions of ``probably reasonable'' scores to both types.\footnote{For example, from a 38-word utterance, \emph{explicit}: ``The minimum wage should be higher than \$7.25''; \emph{implicit}: ``The current minimum wage is insufficient''}

On the conversational Twitter-STS dataset, the method also shows improvement, likely due to the colloquial and contextualized nature of the original utterances.\footnote{Even the ``explicit'' setting generates ``Chris Kelly has died'' from the original ``RIP To tha Mac daddy Chris Kelly''.}
Unsurprisingly, on standard STS benchmarks, the implicit method fares worse, likely because it over-generalizes from specific instances that reduce precision, even if they remain correct: ``A person is mixing a pot of rice.'' $\rightarrow$ ``The person is preparing food.''
Indeed, our method is \emph{intended} to create such generalizations to assist in interpretability at scale, not to improve STS tasks.\footnote{Altering the prompt to support STS by instead generating paraphrases leads to state-of-the-art results, \cref{app:sts}.}

==> Decompositions_as_First_Class_Citizens_arXiv/sections/04-clustering.tex <==
\section{Inferential Decompositions Help Theme Discovery}\label{sec:clustering}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=.89\textwidth]{figures/barplot_clustering_eval.pdf}
    \caption{Human evaluation of clustering outputs. Clusters of decompositions (our method) take significantly less time to review and are more distinctive from one another.
 Relatedness scores are high for the observed comments, but significantly worse membership identification scores reveal this to be a spurious result owed to the topical homogeneity of the dataset (all comments are about COVID vaccines). All differences are significant at $p < 0.05$ except membership scores between comments and sentences and evaluation times for sentences and decompositions.}
    \label{fig:clustering_plot}
    \vspace{-0.3cm}
\end{figure*}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cllll}
\toprule
 $K$ & \textbf{Method} & \textbf{Silhouette}$\uparrow$ & \textbf{CH}$\uparrow$ & \textbf{DB}$\downarrow$ \\
  \midrule
\multirow{3}{*}{15} & Comments             & 0.052           & 247         & 3.41          \\
                    & Sentences            & 0.042           & 219         & 3.74          \\
                    & Decompositions (ours)   & \textbf{0.090}  & \underline{\textbf{329}} & \textbf{3.03} \\  \hline
\multirow{3}{*}{25} & Comments             & 0.035           & 172         & 3.28          \\
                    & Sentences            & 0.035           & 152         & 3.64           \\
                    & Decompositions (ours)   & \textbf{0.096} & \textbf{239} & \textbf{2.80} \\
                    \hline
\multirow{3}{*}{50} & Comments             & 0.029           & 104         & 3.26          \\
                    & Sentences            & 0.042           & 93          & 3.51         \\
                    & Decompositions (ours)   & \underline{\textbf{0.114}} & \textbf{153} & \underline{\textbf{2.73}} \\
\bottomrule
\end{tabular}
}
\caption{Intrinsic metrics of clustering quality. On a random subsample of 10k comments, sentences, and decompositions, the intrinsic metrics rank our model higher both for a fixed number of clusters (bolded) and across clusters (underlined). CH is the Calinski-Harabasz Index and DB is Davies-Bouldin. }
\vspace{-0.3cm}
\label{tab:clustering-intrinsic}
\end{table}


Since the augmented representations we are creating go beyond the observed text to inferentially related propositions, we expect it to be useful in problem settings where observable text is the ``tip of the iceberg'' --- intuitively, problems where it is particularly important to consider not only what was said, but what is \emph{behind} what was said.
Specifically, we ask \emph{whether the representation of comments’ explicit \& implicit propositions lead to improved discovery of themes in a corpus of public opinion.}
Understanding public opinion on a contentious issue fits that description: expressions of opinion are generated from a more complex interplay of personal values and background beliefs about the world. This is a substantive real-world problem; in the US, federal agencies are required to solicit and review public comments to inform policy.%

Our approach is related to efforts showing that intermediate text representations are useful for interpretive work in the computational social sciences and digital humanities, where they can be aggregated to help uncover high-level themes and narratives in text collections \cite{bamman-smith-2015-open, ash2022relatio}. In a similar vein, we cluster inferential decompositions of utterances that express opinion to uncover latent structure analogous to the discovery of narratives in prior work. %
We analyze a corpus of public comments to the U.S Food and Drug Administration (FDA) concerning the emergency authorization of COVID-19 vaccinations in children --- in terms of content and goals, our application resembles the latent argument extraction of~\citet{pacheco-etal-2022-interactively}, who, building on content analysis by \citet{Wawrzuta2021WhatAA}, clustered tweets relating to COVID-19 to facilitate effective annotation by a group of human experts. In our case, we not only discover valuable latent categories, but we are able to assign naturalistic category labels automatically in an unsupervised way.\footnote{In preliminary experiments, topic model outputs were of mixed quality.}


\paragraph{Dataset.} We randomly sampled 10k responses from a set of about 130k responses to a request for comments by the FDA regarding child vaccine authorization.\footnote{\texttt{regulations.gov/document/FDA-2021-N\-1088-0001}. Comments are public and users can elect to post anonymously. We obtained permission from the agency to use these data. We will not directly release the data out of caution, because the original authors did not explicitly consent to redistribution, but we refer interested researchers to \url{https://www.regulations.gov/bulkdownload} and \citet{pampell}. Note that some comments can contain upsetting language, which we communicated to annotators.}  Our dataset contains often-lengthy comments expressing overlapping opinions, colloquial language, false beliefs or assumptions about the content or efficacy of the vaccine, and a general attitude of vaccine hesitancy (see the ``Comment'' column of \cref{tab:fda-exemplars1} for examples).
%

\begin{table*}
    \centering
    \scriptsize{
    \begin{tabular}{p{0.15\textwidth} p{0.25\textwidth} p{0.25\textwidth} p{0.25\textwidth}}
    \toprule
    Source & Cluster 1 & Cluster 2 & Cluster 3 \\ 
    \midrule
    Decomposition Clusters & 
    The vaccine may be harmful to children. \newline 
    Children are vulnerable to the long-term effects of the vaccine. \newline
    Vaccines are still under trials and their side effects are unknown. \newline 
    The vaccine has not been properly tested. \newline 
    There is not enough data on the vaccine's long-term effects. &
    
    Natural immunity is better than vaccine-induced immunity. \newline 
    Natural immunity is important for children to develop. \newline 
    Natural immunity is more effective. \newline 
    Natural immunity is better for fighting the covid virus. \newline 
    People should develop immunities to stay healthy. \newline 
    Natural immunity should be reflected in science. & 

    The government is attempting to control citizens. \newline 
    American rights are being eroded.  \newline 
    The government should investigate the use of \newline  
    We need to protect our children.  \newline 
    The US values freedom and choice.   \\ 
    
\midrule
    Expert Narratives \newline \citet{Wawrzuta2021WhatAA} & 
     The vaccine is not properly tested, it was developed too quickly & 
     Natural methods of protection are better than the vaccine & 
     Lack of trust in the government \\ 
     
\midrule
    Crowdworker Label & 
    Long-term vaccine worries & 
    Natural Immunity & 
    Control by government \\ 

\bottomrule
        
\end{tabular}}
    \caption{For public commentary datasets about COVID-19, clusters of inferential decompositions (our approach, top row) align with arguments discovered independently by \citet{Wawrzuta2021WhatAA} (middle row).
    The overlap is strong despite the commentary coming from different platforms (Government website \& Facebook) and countries (US \& Poland).
    In addition, outside of the exemplars passed to the LLM (\cref{tab:fda-exemplars1}), our approach is also entirely unsupervised.
    In the bottom row, we show an illustrative label for each cluster from a crowdworker.
    }
    \label{tab:cluster_compare}
    \vspace{-0.3cm}
\end{table*}


\paragraph{Method.}
We generate 27,848 unique inferential decompositions from the observable comments at an average of 2.7~per comment.
We use \mbox{$K$-means} clustering to identify categories of opinion, varying $K$.
Specifically, two authors created 31~exemplars from seven original comments from the dataset that exhibit a mixture of implicit proposition types (\cref{tab:fda-exemplars1}). In addition to clustering the observed comments themselves as a baseline, as a second baseline we split each comment into its overt component sentences and cluster the full set of sentences. This results in 10k comments, 45k sentences, and 27k decompositions.

\paragraph{Automated Evaluation.} We lack ground truth labels for which documents belong to which cluster, so we first turn to intrinsic metrics of cluster evaluation: the silhouette \cite{Rousseeuw1987SilhouettesAG}, Calinski-Harabasz \cite{Caliski1974ADM}, and Davies-Bouldin \cite{Davies1979ACS} scores; roughly speaking, these variously measure the compactness and distinctiveness of clusters. Since metrics can be sensitive to the quantity of data in a corpus (even if operating over the same content), we subsample the sentence and decomposition sets to have the same size as the comments (10k).\footnote{Results are similar for the silhouette and Davies-Bouildin scores without subsampling; the Calinski-Harabasz is better for the sentences.}
Clusters of decompositions dramatically outperform clusters of comments and sentences across all metrics for each cluster size---in fact, independent of cluster size, the best scores are obtained by decomposition clusters (Table~\ref{tab:clustering-intrinsic}).

\paragraph{Human Evaluation.} Performance on intrinsic metrics does not necessarily translate to usefulness, so we also evaluate the cluster quality with a human evaluation.
After visual inspection, we set $K=15$.
For a given cluster, we show an annotator four related documents and ask for a free-text label describing the cluster and a 1--5 scale on perceived ``relatedness''. We further perform a membership identification task: an annotator is shown an unrelated distractor and a held-out document from the cluster, and asked to select the document that ``best fits'' the original set of four.
Participant information and other survey details are in \cref{app:survey_details}.

Results are shown in~Fig~\ref{fig:clustering_plot}. While comment clusters receive a higher relatedness score, this is likely due to the inherent topical coherence of the dataset: there are often several elements of similarity between \emph{any} two comments. A lower score in the membership identification task, however, indicates that comment clusters are less distinct. Moreover, the comprehension time for comments is significantly longer than for sentences and decompositions (Evaluation Time in Fig~\ref{fig:clustering_plot}), taking over 50\% longer to read.  On the other hand, clusters of decompositions strike a balance: they obtain moderately strong relatedness scores, can be understood the quickest, and are highly distinct. 

\paragraph{Convergent Validity.} Although further exploration is necessary, we find that our crowdworker-provided labels can uncover themes discovered from classical expert content analysis (\cref{tab:cluster_compare}).
For example, two crowdworkers assign labels containing the text ``natural immunity'' to the cluster in \cref{tab:cluster_compare}---this aligns with the theme \textsc{natural immunity is effective} discovered in \citet{pacheco2023interactive} (through a process requiring more human effort) and a similar narrative in \citet{Wawrzuta2021WhatAA}.
Meanwhile, this concept does \emph{not} appear anywhere in the crowdworker labels for the baseline clusters of sentences or comments.

==> Decompositions_as_First_Class_Citizens_arXiv/sections/05-covote_prediction.tex <==
\section{Decompositions support analyses of legislator behavior}\label{sec:covote_prediction}


Having established our method's ability to facilitate human interpretation of text data (\cref{sec:validation} and \cref{sec:clustering}), we now examine the usefulness of generated inferential decompositions in a very different downstream application where the relevant analysis of text is likely to involve more than just overt language content. %
Here, we model legislator behavior using their speech (here, tweets), asking: \emph{does the similarity between legislators’ propositions help explain the similarity of their voting behavior?}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=.9\textwidth]{figures/topic_41_abortion.pdf}
    \caption{t-SNE \cite{tsne2008} visualization of the embedding space of implicit inferred decompositions found in the ``Abortion'' topic from legislative tweets. $\bigstar$  and \ding{54} are two clusters selected from 10 clusters obtained using $K$-means; $\bigstar$ (59\% Democrat) talks about the role of judiciary in reproductive rights, while the \ding{54} (73\% Republican) talks about banning late stage abortion. Our method leads to more compact (better Silhouette, CH, and DB scores compared to tweets) and easier to interpret clusters that help with narrative discovery.}
    \label{fig:abortion-narratives}
    \vspace{-0.3cm}
\end{figure*}

Traditional theories of homophily \citep{mcpherson2001birds} suggest that shared properties \cite[e.g., electoral geography,][]{clark2013multimember} increase the likelihood that two legislators vote the same way
--- and many research questions have centered around such \emph{co-voting} \citep{Ringe2013,Peng2016, wojcik2018birds}.  In preliminary experiments we found when modeling co-voting, text similarity between legislator was a valuable predictor of co-voting \cite{goel-thesis}. Here we posit that such modeling can further benefit by going beyond surface text to capture inferentially related propositions related to viewpoints.


%

Consider Figure \ref{fig:teaser}.
While the observable tweets themselves are not similar in their surface form, they express similar views regarding the importance of the preservation of nature, something that would be clear to a human reader interpreting them.
This can be captured by inferential decompositions that reveal authors' viewpoints toward the issue. %

We operationalize our method for this purpose by creating exemplars that contain inferences about the utterance topic and perspective (\cref{tab:leg-tweet-exemplars} in appendix). This guides the language model toward domain-relevant facets of similarity between the texts, and therefore the authors of the texts, that may not be apparent from the surface form.





%


\paragraph{Model Setup.} For the task of modeling co-vote behavior, we extend the framework introduced by \citet{Ringe2013} to incorporate individuals' \emph{language} into the model.
At a high level, we operationalize legislator homophily by measuring the similarities of their embedded speech Twitter. 
Following \citet{Ringe2013} and \citet{wojcik2018birds}, we model the log odds ratio of the \emph{co-voting rate} between a pair of legislators $i,j$ using a mixed effects regression model, controlling for the random effects of both actors under consideration.
The co-vote rate $\lambda$ is the number of times the legislators vote the same way --- yea or nay --- divided by their total votes in common within a legislative session.
\vspace{-0.2cm}
\begin{sizeddisplay}{\small}
\begin{align}
    \mathbb{E} \left[
         \log \Big( \frac{\lambda_{ij}}{1 - \lambda_{ij}}
         \Big)
    \right] &=
       \beta_{0} + \bm{\beta}^\top\bm{x}_{ij} + a_{i} + b_{j}
       \label{eq:co_voting_basic}
\end{align}
\end{sizeddisplay}
\noindent $\beta_*$ are regression cofficients, and $a_{i}, b_{j}$ model random effects for legislators $i, j$.\looseness=-1

$\bm{x}_{ij}$ is an $n$-dimensional feature vector, where each element is a similarity score that captures a type of relationship between legislators $i$ and $j$.
While these features have traditionally included state membership, party affiliation, or Twitter connections \citep{wojcik2018birds} or joint press releases \citep{desmarais2015measuring}; we consider the language similarity between pairs of legislators based on our proposed method.


\paragraph{Dataset.}
The goal is to represent each legislator using their language in such a way that we can measure their  similarity to other legislators---our informal hypothesis of the data-generating process is that a latent ideology drives both vote and speech behavior.
Specifically, we follow \citet{vafa-etal-2020-text} by using their tweets; data span the $115^{th}-117^{th}$ sessions of the US Senate (2017--2021).\footnote{Tweets from \url{github.com/alexlitel/congresstweets}, votes from \url{voteview.com/about}.}

We further suppose that ideological differences are most evident when conditioned on a particular issue, such as ``the environment''; in fact, \citet{bateman-lapinski-2017-house} note that aggregated measures like ideal points mask important variation across issues. %
To this end, we first train a topic model on Twitter data to group legislator utterances into broad issues.\footnote{Text was processed using the toolkit from \citet{hoyle-etal-2021-automated}, and modeled with collapsed Gibbs-LDA \cite{Griffiths2004FindingST} implemented in \textsc{Mallet} \cite{mallet}.} 
Two authors independently labeled the topics they deemed most indicative of ideology, based on the top words and documents from the topic-word ($\bm{\beta}^{(k)}$) and topic-document ($\bm{\theta}^{(k)}$) distributions.\footnote{E.g, top words ``border, crisis, biden, immigration'' correspond to the politically-charged issue of immigration; the more benign ``tune, live, watch, discuss'' covers tweets advertising a media appearance to followers. Both annotators initially agreed on 92\% of labels; disagreements were resolved via discussion. The final set of 33 topic-words can be found in \url{github.com/ahoho/inferential-decompositions}.}
Then, for each selected topic $k$ and legislator $l$, we select the top five tweets ${U}^{(k)}_{l} = \{u^{(k)}_{l,1},\ldots u^{(k)}_{l,5}\}$, filtering out those with estimated low probability for the topic, $\theta^{(k)}_{u_l}<0.5$.
Finally, we generate a flexible number of inferential decompositions for the tweets ${R}^{(k)}_l$ using GPT-3.5.\footnote{Results in \cref{tab:covote} are extremely similar when using Alpaca-7B, suggesting the findings are robust.}
We use two prompts each containing six different exemplars to increase the diversity of inferences.
The collections of tweets and decompositions are then embedded with Sentence-Transformers \cite[\texttt{all-mpnet-base-v2} from][]{reimers-gurevych-2019-sentence}. 

\paragraph{Language Similarity.} To form a text-based similarity measure between legislators $i$ and $j$, we first compute the pairwise cosine similarity between the two legislators' sets of text embeddings, $s_\text{cos}\left({U}^{(k)}_{i} \times {U}^{(k)}_{j}\right)$ (or ${R}$ for the decompositions).
The pairs of similarities must be further aggregated to a single per-topic measure; we find the $10^{\text{th}}$ percentile works well in practice (taking a maximum similarity can understate differences, whereas the mean or median overstates them, likely due to finite sample bias; see \citealt{demszky-etal-2019-analyzing}).
This process creates two sets of per-topic similarities for each $(i,j)$-legislator pair, $s^{(k)}_{ij}(u), s^{(k)}_{ij}(r)$. 



\begin{table}[!t]
\captionsetup{font=footnotesize}
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{@{}lr|rr|rr@{}}
\toprule
\multicolumn{1}{c}{\textit{\textbf{}}} &
  \multicolumn{1}{c|}{\textit{\textbf{$\bm{115^{th}}$}}} &
  \multicolumn{2}{c|}{\textit{\textbf{$\bm{116^{th}}$}}} &
  \multicolumn{2}{c}{\textit{\textbf{$\bm{117^{th}}$}}} \\[0.2cm] 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$\bm{\hat{\beta}}\uparrow$ \end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$\bm{\hat{\beta}}\uparrow$ \end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{MAE}$\downarrow$%
  \end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$\bm{\hat{\beta}}\uparrow$ \end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{MAE}$\downarrow$%
  \end{tabular}} \\ \midrule
Sim. $U$
   &
  $10.64$ &
  $11.86$ &
  $744.81$ &
  $17.36$ &
  $981.56$ \\ \midrule[0.25pt]
Sim. $R$
   &
  $12.69$ &
  $17.31$ &
  $736.21$ &
  $23.0$ &
  $964.86$ \\ \midrule[0.25pt]
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\underset{+}{\text{Sim. }U}$\\Sim. $R$\end{tabular}} &
  $\underset{\phantom{+}}{6.02}$ &
   $\underset{\phantom{+}}4.40$ &
  \multirow{2}{*}{$741.59$} &
   $\underset{\phantom{+}}11.09$ &
  \multirow{2}{*}{$935.45$} \\
 &
  $7.01$ &
  $12.67$ &
   &
  $10.82$ &
   \\\bottomrule
\end{tabular}}
\caption{Explanatory power ($\hat{\beta}$) and predictive capacity (\textbf{MAE}) of text similarity measures in a mixed effects model of co-vote behavior for 3 sessions of the US Senate. Coefficients are large and significantly above zero ($p<0.001$). For the mean absolute error (MAE), we multiply the predicted co-vote agreement error with the total number of votes in common for the legislator pair. %
}
\vspace{-0.3cm}
\label{tab:covote}
\end{table}

\paragraph{Results.} Similarities based on inferential decompositions, $s_{ij}(r)$, both help explain the variance in co-vote decisions as well as help predict co-voting agreement over and above similarities based on the observed utterances (tweets) alone, $s_{ij}(u)$ (\cref{tab:covote}).\footnote{We use membership in the same political party as a control variable in each of the mixed effects models.}
Specifically, for the regression models, across three Senate sessions, the mixed effects model that uses similarity in decompositions ($R$; row 2 in \cref{tab:covote}) has a higher regression coefficient ($\hat{\beta}$) than the corresponding coefficient for similarity in utterances ($U$; row 1). 
This also holds for a model that uses both similarity measures in the regression (row 3).

\begin{figure*}[tb]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/incorrect_correct_far_close.pdf}
    \caption{
    Pairs of legislative tweets (green) and associated decompositions (orange).
    Here, we show instances where embeddings of the decompositions are \emph{closer} than embeddings of the original tweets.
    The example on the left shows the method working as intended, whereas the example on the right is undesired behavior.
    Although the method generates multiple decompositions per tweet, we only show the two closest.
    In \cref{app:leg-tweet-analysis}, we discuss instances where the decompositions are \emph{more distant} than the tweets.
}
    \label{fig:legislative-tweet-analysis-far-close}
    \vspace{-0.3cm}
\end{figure*}

Additionally, we compare the predictive capacity of the two similarity measurements in two scenarios: we train the model on data from the $115^{th}$ Senate to predict co-vote for the $116^{th}$, and train on data from the $115^{th}$ and $116^{th}$ sessions to predict co-vote for the $117^{th}$.
Using similarity in decompositions leads to a lower MAE between predicted and actual co-vote agreement than using similarity in utterances; both similarity measures together further reduce the error for the $117^{th}$ Senate (\cref{tab:covote}). 

Examples of utterances and their decompositions in \cref{fig:legislative-tweet-analysis-far-close} help contextualize these results.
For the left-hand example, the method infers a shared implicit proposition---``President Trump is weak''---that underlies two tweets with little \emph{observed} text in common.
However, the method can occasionally overstate similarities between utterances (and thus, between legislators): while the decompositions in the right-hand example are valid inferences, they are also \emph{overly general} (``voting is important'').

Our approach further uncovers the narratives that emerge among legislators from different parties around a particular issue. In discussions around abortion and reproductive health, our decompositions capture fine-grained viewpoints about the role of supreme court and judiciary, and the contentious debate around late stage abortions (Fig. \ref{fig:abortion-narratives}). Clustering over implicit decompositions reveal finer opinion-spaces that succinctly capture author viewpoints towards facets of a particular issue.






==> Decompositions_as_First_Class_Citizens_arXiv/sections/06-conclusion.tex <==
\section{Related Work}

As a computational text analysis method that operates over reduced representations of text data, our work is similar to that of \citet{ash2022relatio} and \citet{bamman-smith-2015-open}. Closest to our clustering effort (\cref{sec:clustering}), ~\citet{ernst-etal-2022-proposition} extract and cluster paraphrastic propositions to generate summaries. 
However, they constrain themselves to the observed content alone, limiting their ability to capture context-dependent meaning.

Our method continues the relaxation of formal semantic representations in NLP, a process exemplified by the Decompositional Semantics Initiative \cite{white-etal-2016-universal}, which aims to create an intuitive semantic annotation framework robust to variations in naturalistic text data.
The generated inferential decompositions in our work are human-readable and open-ended, structured by a user-defined schema in the form of exemplars.
In this way, we also follow a path forged by natural language inference \cite{bowman-etal-2015-large,chen-etal-2017-enhanced}, which has increasingly relaxed semantic formalisms when creating datasets. 
In future work, we plan to relate both the exemplars and outputs to formal categories and investigate their utility in downstream tasks.

Our methods for generating decompositions are distinct from \emph{extracting} commonsense knowledge from text---e.g., through templates \cite{Tandon_Melo_Weikum_2014}, free-form generation from LLMs \citet{bosselut-etal-2019-comet}, or script induction \cite{schank1975} (which can also use LLMs, \citealt{sancheti-rudinger-2022-large}).
Our decompositions are not designed to produce general commonsense knowledge such as ``rain makes roads slippery'' \cite{sap-etal-2020-commonsense}, but instead to surface the explicit or implicit propositions inferrable from an utterance.

Our work also bears a similarity to \citet{opitz-frank-2022-sbert}, who increase the interpretability of sentence embeddings using an AMR graph for a sentence.
However, AMR graphs are also tied to the information present in an utterance's surface form (and, moreover, it is unclear whether AMR parsers can accommodate noisier, naturalistic text).

LLMs have been used to generate new information ad-hoc in other settings, for example by augmenting queries \cite{Mao2020GenerationAugmentedRF} or creating additional subquestions  in question-answering \cite{Chen2022GeneratingLA}. 
In contemporaneous work, \citet{ravfogel2023retrieving} use an LLM to generate abstract descriptions of text to facilitate retrieval.
In ~\citet{gabriel-etal-2022-misinfo}, the authors model writer intent from a headline with LLMs. ~\citet{becker-etal-2021-reconstructing} generate implicit knowledge that conceptually connects contiguous sentences in a longer body of text.


\section{Conclusion}\label{sec:future_work}

Our method of inferential decompositions is useful for text-as-data applications.
First, we uncover high-level narratives in public commentary, which are often not expressed in surface forms.
Second, we show that, by considering alternative representations of legislators' speech, we can better explain their joint voting behavior.
More broadly, treating implicit content as a first-class citizen in NLP---a capability enabled via generation in large language models---has the potential to transform the way we approach problems that depend on understanding what is behind people's utterances, rather than just the content of the utterances themselves.

 


==> Decompositions_as_First_Class_Citizens_arXiv/sections/08-limitations.tex <==
\section{Limitations}\label{sec:limitations}
Our validity checks in Section \ref{sec:validation} reveal that while most decompositions are deemed reasonable by humans, some are not (Fig. \ref{fig:validation}.).
It remains to be studied the extent to which implausible generations are affecting with the results, or if they are introducing harmful propositions not present in the original text.
In future work, we will explore whether known political biases of language models \cite{Santurkar2023WhoseOD} affect our results.
Although an open-source model (specifically Alpaca-7B \citealt{alpaca}) produces similar results to those reported, our main experiments primarily use models released by OpenAI, which may lead to potential reproducibility issues.
All our analyses and experiments focus on utterances in the English language, which could limit the generalizability of our method.
Relatedly, our experiments are also specific to the US sociocultural context and rely on models that are known to be Western-centric \cite{palta-rudinger-2023-fork}. 

The embeddings could be made more sensitive to the particular use case. In future work, we plan to additionally fine-tune the embeddings so that they are more sensitive to the particular use case \cite[e.g., establishing argument similarity,][]{Behrendt2021ArgueBERTHT}).

==> Decompositions_as_First_Class_Citizens_arXiv/sections/09-ethics-statement.tex <==
\section{Ethics Statement}
The work is in line with the ACL Ethics Policy. Models, datasets, and evaluation methodologies used are detailed throughout the text and appendix. The human evaluation protocol was approved by an institutional review board. No identifying information about participants was retained and they provided their informed consent. We paid per survey based on estimated completion times to be above the local minimum wage (\cref{app:survey_details}). Participants were paid even if they failed attention checks. All the datasets were used with the appropriate or requested access as required. We acknowledge that we are using large language models, which are susceptible to generating potentially harmful content.

Generally, the potential for misuse of this method is not greater than that of the large language models used to support it. In theory, it is possible that a practitioner could draw incorrect conclusions about underlying data if the language model produces a large number of incorrect statements. To the extent that those conclusions inform downstream decisions, there could be a potential for negative outcomes. For this reason, we advocate for manual verification of a sample of outputs in sensitive contexts (step 4 of our protocol \cref{sec:background}).

==> Decompositions_as_First_Class_Citizens_arXiv/sections/10-acknowledgements.tex <==
\section{Acknowledgements}

We thank Sweta Agrawal for her abundant support and feedback on earlier drafts and Justin Pottle for assistance with data quality annotation. We also appreciate productive discussions with both Rachel Rudinger and Maharshi Gor, Jordan Boyd-Graber and Chenglei Si gave excellent notes during our internal paper clinic, and we thank our anonymous reviewers for their very helpful comments. This work was supported in part by the National Science Foundation under award \#2008761, the Food and Drug Administration (FDA) of the U.S. Department of Health and Human Services (HHS) as part of a financial assistance award (Center of Excellence in Regulatory Science and Innovation cooperative agreement U01FD005946 with the University of Maryland), and a grant from the University of Maryland Social Data Science Center. Any opinions, findings, conclusions, or recommendations expressed in this material are those of the authors and do not necessarily represent the official views of, nor an endorsement, by any sponsor or by the U.S. government. 




